T5-SR: A Unified Seq-to-Seq Decoding Strategy for Semantic Parsing

Translating natural language queries into SQLs in a seq2seq manner has attracted much attention recently. However, compared with abstract-syntactic-tree-based SQL generation, seq2seq semantic parsers face much more challenges, including poor quality on schematical information prediction and poor semantic coherence between natural language queries and SQLs. This paper analyses the above difficulties and proposes a seq2seq-oriented decoding strategy called SR, which includes a new intermediate representation SSQL and a reranking method with score re-estimator to solve the above obstacles respectively. Experimental results demonstrate the effectiveness of our proposed techniques and T5-SR-3b achieves new state-of-the-art results on the Spider dataset.

==> case_table.tex <==
\begin{tabular}{ll}
\toprule
\textbf{Query:}                                                    & Find number of pets owned by students who are older than 20.                                                                                                                                    \\ \specialrule{0em}{1pt}{1pt}
\textbf{Gold:}                                                     & \begin{tabular}[c]{@{}l@{}}SELECT count ( * ) FROM student AS T1 JOIN has\_pet AS T2 ON T1.stuid = T2.stuid WHERE \\ T1.age \textgreater 20\end{tabular}                                        \\ \specialrule{0em}{1pt}{1pt}
\textbf{SSQL:}                                                     & SELECT count ( * ) FROM student , has\_pet WHERE student.age \textgreater 20                                                                                                                    \\ \specialrule{0em}{1pt}{1pt}
\textbf{T5:}                                                       & \begin{tabular}[c]{@{}l@{}}SELECT count ( * ) FROM \red{has\_pet AS T1 JOIN pets AS T2 ON T1.petid = T2.petid JOIN student} \\ \red{AS T3 ON T1.stuid = T3.stuid} WHERE T3.age \textgreater 20\end{tabular} \\ \specialrule{0em}{1pt}{1pt}
\textbf{T5-SR:}                                                    & \begin{tabular}[c]{@{}l@{}}SELECT count ( * ) FROM \green{student AS T1 JOIN has\_pet AS T2 ON T1.stuid = T2.stuid} WHERE \\ T1.age \textgreater 20\end{tabular}                                        \\ \hline
\textbf{Query:}                                                    & How many models does each car maker produce? List maker full name, id and the number.                                                                                                           \\ \specialrule{0em}{1pt}{1pt}
\textbf{Gold:}                                                     & \begin{tabular}[c]{@{}l@{}}SELECT T1.FullName , T1.Id , count ( * ) FROM car\_makers AS T1 JOIN model\_list AS T2 ON \\ T1.Id = T2.Maker GROUP BY T1.Id\end{tabular}                            \\ \specialrule{0em}{1pt}{1pt}
\textbf{SSQL:}                                                     & \begin{tabular}[c]{@{}l@{}}SELECT car\_makers.FullName , car\_makers.Id , count ( * ) FROM car\_makers , model\_list \\ GROUP BY car\_makers.Id\end{tabular}                                    \\ \specialrule{0em}{1pt}{1pt}
\textbf{T5:}                                                       & \begin{tabular}[c]{@{}l@{}}SELECT T1.FullName , \red{T1.Maker} , \red{T1.FullName} FROM car\_makers AS T1 JOIN model\_list AS \\ T2 ON T1.Id = T2.Maker GROUP BY T1.Id\end{tabular}                         \\ \specialrule{0em}{1pt}{1pt}
\textbf{T5-SR:}                                                    & \begin{tabular}[c]{@{}l@{}}SELECT T1.FullName , \green{T1.Id} , \green{count ( * )} FROM car\_makers AS T1 JOIN model\_list AS T2 ON \\ T1.Id = T2.Maker GROUP BY T1.Id\end{tabular}                            \\ \specialrule{0em}{1pt}{1pt}
%\textbf{\begin{tabular}[c]{@{}l@{}}T5-SSQL\\ Beam 1:\end{tabular}} & \begin{tabular}[c]{@{}l@{}}SELECT T1.FullName , \red{T1.Maker} , count ( * ) FROM car\_makers AS T1 JOIN model\_list AS T2 \\ ON T1.Id = T2.Maker GROUP BY T1.Id\end{tabular}                         \\
\bottomrule
\end{tabular}
